A novel reliability attack of Physical Unclonable Functions

Physical Unclonable Functions (PUFs) are emerging as promising security primitives for IoT devices, providing device fingerprints based on physical characteristics. Despite their strengths, PUFs are vulnerable to machine learning (ML) attacks, including conventional and reliability-based attacks. Conventional ML attacks have been effective in revealing vulnerabilities of many PUFs, and reliability-based ML attacks are more powerful tools that have detected vulnerabilities of some PUFs that are resistant to conventional ML attacks. Since reliability-based ML attacks leverage information of PUFs' unreliability, we were tempted to examine the feasibility of building defense using reliability enhancing techniques, and have discovered that majority voting with reasonably high repeats provides effective defense against existing reliability-based ML attack methods. It is known that majority voting reduces but does not eliminate unreliability, we are motivated to investigate if new attack methods exist that can capture the low unreliability of highly but not-perfectly reliable PUFs, which led to the development of a new reliability representation and the new representation-enabled attack method that has experimentally cracked PUFs enhanced with majority voting of high repetitions.

==> sec2_PUF_bckgrounds.tex <==
%\section{Introduction}
%Physically Unclonable Functions (PUFs) have emerged as a promising security primitive for low-cost and low-power Internet-of-Things (IoT) devices.  By providing devices with unique fingerprints derived from their inherent physical characteristics, PUFs offer a new approach to implementing authentication and encryption. The foundational concept behind PUFs is to move away from the conventional practice of storing keys in non-volatile memories (NVMs). Not only because such memories are costly, but they are also vulnerable to specific attacks, such as cold boot attacks \cite{halderman2009lest}, especially when the IoT devices are widely accessible. 

%Instead of retrieving keys from NVMs, PUFs utilize inherent physical variations as devices' unique ``fingerprints''. These fingerprints, arising from minute inconsistencies during manufacturing processes, are physically unclonable and distinct for each device. This inherent uniqueness is utilized to generate digital identifiers, and these identifiers can serve as a robust defense mechanism against potential security threats, including impersonation and counterfeiting, prevalent in IoT devices \cite{guajardo2007fpga,ruhrmair2009foundations,maes2010physically}. PUFs have been extensively studied in recent years \cite{lee2004technique, lim2004extracting,gassend2002controlled,gassend2002silicon,tuyls2007security}. Due to their resilience against physical clones, no requirement of secure memory for key storage, and their cost-effective hardware implementation, PUFs hold the potential to overcome challenges that conventional cryptographic methods face in the IoT landscape. \par

%Despite their resilience against physical cloning, PUFs are not immune to vulnerabilities, and a thorough understanding of all potential weaknesses is crucial. PUFs face a spectrum of threats, including side-channel-based modeling attacks and CRP-based based modeling attacks \cite{ruhrmair2013puf, aseeri2018machine, santikellur2019deep, majzoobi2008lightweight, alkatheiri2017towards, wisiol2022neural, mursi2020fast, thapaliya2021machine}, where CRP denotes challenge-response-pair. 

%CRP-based modeling attacks include conventional and reliability-based machine learning (ML) attacks. While some PUFs with sophisticated architectures can resist conventional ML attacks, reliability-based ML attacks have demonstrated success in compromising many PUFs that conventional methods cannot breach \cite{becker2015gap,6581579}.  Reliability-based attacks exploit the variability in PUF responses, by applying the same challenges repeatedly to the PUF to get multiple responses for each challenge and analyzing the responses to uncover exploitable patterns.  Since PUFs inherently process some level of unreliability, the risk of susceptibility to reliability-based attacks is real, even for PUFs engineered to withstand conventional machine learning assaults. Resistance to reliability-based modeling attacks is also an important metric for evaluating PUF designs.

%Some PUF attacks methods use side-channel information, including power consumption [x10-x13], electromagnetic waves [x14], photonic emission [x15], signal timing or frequency [x12,x16], etc. to help predict PUFs' responses. There have been many successful efforts on fighting side-channel attacks, including dynamic voltage scaling [x17,x18], balanced gates [x10,x19], converter reshuffling [x20,x21]. Some side-channel attack methods use reliability information together with other side-channel information [xx]. In this paper we consider attacks using only reliability information.

%[x10]	A. Mahmoud, U. Rűhrmair, Mehrdad Majzoobi, F. Koushanfar, "Combined modeling and side channel attacks on strong PUFs", Cryptology ePrint Archive Report 2013/632, 2013.
%[x11]	U. Rűhrmair, X. Xu, J. Sőlter, A. Mahmoud, F. Koushanfar, W. Burleson, "Power and timing side channels for PUFs and their efficient exploitation", International Workshop on Cryptographic Hardware and Embedded Systems (CHES2014). Lecture Notes in Computer Science, vol 8731. 2014, Springer, Berlin, Heidelberg.
%[x12]	Sheng Wei, J. B. Wendt, A. Nahapetiany, M. Potkonjak, "Reverse Engineering and Prevention Techniques for Physical Unclonable Functions Using Side Channels".  Proc. 51st Annual Design Automation Conference (DAC '14), June 2014, San Francisco, California, pp.1–6.
%[x13]	G. T. Becker and R. Kumar, "Active and passive side-channel attacks on delay based PUF designs", IACR Cryptology ePrint Archive, 287. 2014.
%[x14]	Dominik Merli, Johann Heyszl, Benedikt Heinz, Dieter Schuster, Frederic Stumpf, and Georg Sigl, "Localized electromagnetic analysis of RO PUFs". IEEE International Symposium on Hardware-Oriented Security and Trust (HOST), June 2013, Austin, Texas.
%[x15]	S. Tajik, E. Dietz, S. Frohmann, et al. "Photonic Side-Channel Analysis of Arbiter PUFs". J Cryptol, Vol. 30, pp. 550–571 (2017).
%[x16]	X. Xu and W. Burleson, "Hybrid side-channel/machine-learning attacks on PUFs: a new threat?", Proc. Conference on Design, Automation and Test in Europe (DATE '14),  March 2014, Article No.: 349, pp. 1–6.
%[x17]	S. Yang, W. Wolf, N. Vijaykrishnan, D. N. Serpanos and Yuan Xie, "Power attack resistant cryptosystem design: a dynamic voltage and frequency switching approach," Design, Automation and Test in Europe, 2005, pp. 64-69 Vol. 3.
%[x18]	N.D.P. Avirneni and A. K. Somani, "Countering Power Analysis Attacks Using Reliable and Aggressive Designs," in IEEE Transactions on Computers, vol. 63, no. 6, pp. 1408-1420, June 2014.
%[x19]	W. Yu and Y. Wen, “Leveraging Balanced Logic Gates as Strong PUFs for Securing IoT Against Malicious Attacks,” J. Electronic Testing: Theory and Applications, vol. 35, no. 6, pp. 853-865, December 2019.
%[x20]	W. Yu and S. Köse, “Time-Delayed Converter-Reshuffling: An Efficient and Secure Power Delivery Architecture,” IEEE Embedded Systems Letters, vol. 7, no. 3, pp. 73-76, September 2015.
%[x21]	W. Yu and S. Köse, “Charge-Withheld Converter-Reshuffling (CoRe): A Countermeasure Against Power Analysis Attacks,” IEEE Transactions on Circuits and Systems II: Express Briefs, vol. 63, no. 5, pp. 438-442, May 2016.

%Since there are many techniques [] developed for improving the reliability of PUFs, it is natural to think if reliability-enhancing techniques can also be used to fight reliability-based ML attacks, or conversely, if existing reliability-based ML attacks will remain effective in compromising highly reliable PUFs. This points to a notable research gap, a gap on the feasibility of building defense using reliability enhancing techniques. 

%To address this gap, we start our investigation first buy exploring the effectiveness of current reliability-based attacks on high-reliability PUFs. Majority-voting is a simplistic reliability-enhancing technique, and we decide to test it on PUFs that have succumbed to existing reliability-based ML attacks. We implemented PUFs on FPGAs and applied majority-voting to PUF responses with different repeats of majority-voting. Then, reliability-based ML attacks were applied to responses out of majority-voting enhanced PUFs. In the study, we discover that attack methods exhibit decreasing attack power as PUF reliability increases and completely ceased to be effective when majority voting uses 50 or more repeats. This discovery, first identified in our study, renders majority-voting as a simple and effective defense tool against existing RbML attacks. But we are immediately tempted to ponder if highly reliable PUFs are truly secure against reliability-based ML or waiting for another more potent attack method to emerge. 

%With this pondering, we started to examine current reliability-based ML attack methods and believe that, for a group of most broadly applicable methods, the representation of reliability information is the underlying factor for the failure of these methods for high reliability PUFs. With their reliability representation, the dimensionality of the output of a machine learning method grows with the reliability of the PUF, and eventually destroys the learning power of the method when the reliability, and consequently the dimensionality, becomes too high. In an attempt to develop new reliability-based ML attack methods for high reliability PUFs, we introduce a novel approach to representing PUF reliability, an approach emphasizing low output dimensionality. We developed two representations of this approach, which have provided machine learning methods substantially improved learning power for attacking highly reliable PUFs. Thus, the main contributions of this paper are 
%\begin{enumerate}
%    \item the discovery that majority voting provides effective defense against existing reliability-based ML attack methods, and 
%    \item the development of new representations of PUF reliability information, which enable machine learning methods to successfully attack high reliability PUFs.
%\end{enumerate}
%The remainder of the paper is organized as follows.  ... HERE



\section{Background on Arbiter PUF and its variants}
In order to help technical discussions in later sections, we will briefly describe the Arbiter-PUF, XOR-Arbiter-PUF, Interpose-PUF, and Feed Forward PUF in this subsection.

%\subsection{Arbiter PUF}
An n-bit arbiter PUF, shown in Figure \ref{f1}, consists of n stages, each containing two multiplexers (MUXs). When a rising signal is applied, it enters the arbiter PUF at the first stage and splits into two signals. These two signals are then routed through gates at each stage, with the propagation paths at each stage determined by the challenge bit. Finally, the two signals reach a D flip-flop, which serves as an arbiter to determine whether the signal on the top path or the signal on the bottom path arrives first. If the top path signal arrives first, the D flip-flop returns a response of 1, and if the bottom path signal arrives first, the D flip-flop returns a response of 0.

 \begin{figure}
%        \centering
        \includegraphics[width=8.5cm]{1.png}
        \caption{An arbiter PUF with n bits of challenge.}
        \label{f1}
\end{figure}


    
\subsection{XOR-Arbiter-PUF}
The XOR-arbiter-PUF (XOR-PUF) In \cite{suh2007physical} was proposed to overcome the susceptibility of arbiter PUFs to machine learning attacks. The \emph{k}-XOR-PUF utilizes a \emph{k}-input XOR gate to combine the responses of $k$ arbiter PUFs to generate the final response. An XOR-PUF example is shown in Figure \ref{f2}.

 \begin{figure}
       \centering
        \includegraphics[width=8cm]{2_1.png}
        \caption{Illustration of an XOR-PUF with n arbiter PUF components; the final response is the XORed result of n arbiter-PUF responses.}
        \label{f2}
\end{figure}
\subsection{Interpose-PUF}

 \begin{figure}
%        \centering
        \includegraphics[width=9.5cm]{3.png}
        \caption{Schematic representation of Interpose PUFs.}
        \label{f3}
\end{figure}

Nguyen et al. \cite{nguyen2019interpose} introduced the Interpose-PUF (IPUF) that utilizes a domino structure to resist reliability-based machine-learning attacks without the need for countermeasures at the protocol level. The IPUF comprises two XOR Arbiter PUFs, namely the x-(upper) and y-(lower) PUF. The x-XOR PUF response serves as an additional challenge bit for the y-XOR PUF. The authors argue that the constituent APUFs of the x-XOR PUF cannot be accurately modeled by reliability attacks, based on their security analysis.

 \subsection{Feed Forward Arbiter PUF and Feed Forward XOR Arbiter PUF}

 \begin{figure}
 \centering
     \includegraphics[width=89mm]{ff.png}
 \caption{Schematic representation of Feed Forward Arbiter PUFs.}
 \label{f4}
 \end{figure}

 Introduced to improve resistance against modeling attacks \cite{gassend2004identification}, the Feed Forward Arbiter PUF (FF-PUF) adds feed-forward loops to the APUF (see Fig.\,\ref{f4} for illustration of an FF-PUF with a single feed-forward loop), whereby the response from one stage influences the decisions in subsequent stages. In a Feed-Forward XOR Arbiter PUF (FF-XOR-PUF)\cite{avvaru2019feed}, multiple FF-PUFs are evaluated in parallel, and the XOR of the response bits of FF-PUFs is returned as the final output of the PUF.


==> sec_HARA.tex <==
\section{Hierarchical and Aggregated Reliability Representation Method}

\subsection{Natural Solution to Address the "Curse of Dimensionality"}

 Confronted with the challenges of high dimensionality inherent in traditional methods, a logical initial step was to reduce the dimensionality of reliability vectors. A straightforward strategy adopted was the rounding method, which aimed to condense the results into a more manageable representation. For example, from a set of 1000 measurements, this method would round the data to produce an effective 10 output nodes.

Confronted with the curse of dimensionality in traditional reliability representation methods, there is a pressing need for innovative approaches that efficiently manage data complexity. A straightforward strategy adopted was the rounding method, which aimed to condense the results into a more manageable representation. For example, "Rounding\_1000\_10" denotes from a set of 1000 measurements, this method would round the data to produce an effective 10 output nodes. While this approach successfully reduced data volume, it fell short in retaining the nuanced details of reliability information, a shortfall critically pronounced in the analysis of high-reliability PUFs.

\begin{table*}[htbp]
\centering
\caption{Results of Attacks on 64-bit 10-XOR-PUFs and (1,8)-iPUFs Applied with Majority Voting Using the Rounding Method}
\label{puf_combined_rounding}
\linespread{1.3}\selectfont
\setlength\tabcolsep{5pt}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{PUF Type} & \textbf{Num\_MV} & \textbf{Attack\_Method} & \textbf{Training Size(Unique)} & \textbf{Success Rate} \\ \hline
\multirow{6}{*}{\textbf{10-XPUF}}    & \multirow{2}{*}{5}  & Rounding\_1000\_10  & 1m & 90\% \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 80\% \\ \cline{2-5} 
                                     & \multirow{2}{*}{20} & Rounding\_1000\_10  & 1m & 30\% \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 35\% \\ \cline{2-5} 
                                     & \multirow{2}{*}{50} & Rounding\_1000\_10  & 1m & 5\%  \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 0\%  \\ \hline
\multirow{6}{*}{\textbf{(1,8)-iPUF}} & \multirow{2}{*}{5}  & Rounding\_1000\_10  & 1m & 80\% \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 60\% \\ \cline{2-5} 
                                     & \multirow{2}{*}{20} & Rounding\_1000\_10  & 1m & 40\% \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 40\% \\ \cline{2-5} 
                                     & \multirow{2}{*}{50} & Rounding\_1000\_10  & 1m & 0\%  \\ \cline{3-5} 
                                     &                     & Rounding\_1000\_100 & 1m & 0\%  \\ \hline
\end{tabular}
\end{table*}

Our experimental results in Table~\ref{puf_combined_rounding} revealed that the rounding method exhibited improved performance compared to prior methods. However, the limitations of this method became apparent, particularly in terms of information loss. This shortfall highlighted the necessity for a more sophisticated solution — one that not only reduces data complexity but also ensures that the intricate nuances of reliability data are not lost in the process.

\subsection{Proposed Hierarchical and Aggregated Reliability Representation Method}

Reflecting on the discussions about the SLMSA and MLMSA methods in the related work section, and the observations from the previous subsection, it becomes evident that the performance of machine learning models in reliability-based attacks on PUFs is profoundly influenced by the representation of reliability information. The MLMSA method, for instance, employs distinct representations for different outputs, as opposed to the mixed output approach in the SLMSA method. This separation of outputs leads to a reduction in data dimensionality, enhancing model performance. However, this approach to reliability representation still encounters the "Curse of Dimensionality" when applied to high-reliability PUFs. Notably, this challenge is not exclusive to these methods; even the ALSCA method, which utilizes the same reliability representation, faces the same dimensional complexities in the context of high-reliability PUFs.


Our initial response to this challenge, the "rounding" method, aimed to tackle the issue of high dimensionality by simplifying the reliability information into a more condensed representation. While this method showed a marked improvement in performance compared to its predecessors, it was hampered by an unavoidable loss of information, which proved to be a significant limitation, particularly for high-reliability PUFs.

This realization underscored the need for a more advanced and effective approach to represent reliability information. Our objective became twofold: to reduce the complexity of high-dimensional data while ensuring the retention of essential reliability details. In response to this, we developed the Hierarchical and Aggregated Reliability Representation (HARR) method. HARR stands out by adeptly reducing data complexity and preserving detailed reliability information, achieving both goals without compromising one for the other. This method represents a significant stride forward in the field of reliability representation for PUFs, promising enhanced performance in machine learning-based security analyses.


\textbf{Hierarchical Measurement:}
The foundation of the HARR method lies in its detailed, iterative sampling process for each PUF challenge. Unlike conventional methods or the rounding method, which may overlook subtle variations, HARR delves deeply into each response. This primary phase meticulously collects comprehensive reliability metrics, ensuring that even the most nuanced aspects of PUF behavior are captured. 


\textbf{Aggregated Representation:}
The innovation extends to how HARR handles the data post-collection. The subsequent aggregated representation phase synthesizes the detailed data from the hierarchical phase into a comprehensive overview. This stage is instrumental in revealing broader reliability patterns and trends, transforming complex data sets into coherent, insightful summaries. Multiple rounds of analysis in this phase provide a macro-level understanding of the PUF's reliability, encapsulating the essence of the data without the burden of its complexity.


The Hierarchical and Aggregated Reliability Representation method emerges as a comprehensive solution, addressing the limitations of existing reliability representation methods. By adopting a dual approach that emphasizes both dimensionality reduction and information retention, HARR offers a nuanced and efficient strategy for analyzing high-reliability PUFs. The following outlines the distinct steps involved in the HARR method:


\begin{enumerate}
    \item \textbf{Initial Sampling:} 
    For each Challenge-Response Pair, the process is repeated $N$ times, akin to traditional methods. The number of '0' and '1' responses are counted to establish a primary reliability measure.
    
    \item \textbf{Aggregated Reliability Sampling:} 
    The initial sampling process is repeated $(m-1)$ times, resulting in $M$ reliability measures, each derived from $N$ CRP repetitions. These measures capture inherent variability and unreliability in responses.
    
    \item \textbf{Reliability Distribution Array:} 
    An array of length $N+1$ is created, with each index corresponding to a possible reliability measure (from 0 to $N$ '1' responses out of $N$ CRP repetitions). The array is incremented based on the accumulated $M$ reliability measures.
    
    \item \textbf{Probability Distribution Synthesis:} 
    This final step transforms the accumulated counts in the reliability distribution array into a probability distribution. By dividing each count in the array by the total number of measures $M$, we synthesize a probability distribution over the $N+1$ possible reliability measures. This distribution offers a refined and insightful portrayal of the PUF's reliability, capturing the subtleties and complexities inherent in high-reliability contexts.

\end{enumerate}

The algorithmic foundation of the HARR method, as presented in Algorithm~\ref{alg:reliability-assessment}, is more than a procedural flow; it encapsulates the essence of our innovative approach to reliability assessment. This algorithm is carefully designed to ensure that each step contributes meaningfully to the overall reliability analysis, providing a nuanced and comprehensive understanding of PUF behavior.

\begin{figure*}
\centering
    \includegraphics[width=15cm]{HARR.jpg}
\caption{Illustration of the reliability representation of the proposed HARR method.}
\label{HARR}
\end{figure*}

\begin{algorithm}
\caption{Hierarchical and Aggregated Reliability Representation}
\label{alg:reliability-assessment}
\begin{algorithmic}[1]
\Procedure{HierarchicalReliability}{$Challenge$}
\State \textbf{Input:} Challenge
\State \textbf{Output:} Probability distribution of reliability measures
\State \textbf{Parameters:} $N$, $M$.
\State $reliabilityCounts \gets$ array of size $N+1$ initialized to zeros.

\For{$i = 1$ to $M$}
    \State $responses \gets$ Repeat $Challenge$ $N$ times
    \State $r \gets$ Count of '1' in $responses$
    \State $reliabilityCounts[r] \gets reliabilityCounts[r] + 1$
\EndFor

\State $probabilityDistribution \gets$ $reliabilityCounts/ M$
\State \Return $probabilityDistribution$
\EndProcedure
\end{algorithmic}
\end{algorithm}

As we progress, the subsequent sections will delve into the empirical validation of the HARR method. Through rigorous testing and analysis, we aim to demonstrate its effectiveness and potential as a significant advancement in PUF security research. In the following section, we will evaluate the effectiveness of this HARR approach through a series of experiments, examining if, and how much, improvement in high-reliability PUF modeling performance can be attained with our HARR method.

